Amplitude Retrieval for Channel Estimation of MIMO Systems with One-Bit ADCs

This letter revisits the channel estimation problem for MIMO systems with one-bit analog-to-digital converters (ADCs) through a novel algorithm--Amplitude Retrieval (AR). Unlike the state-of-the-art methods such as those based on one-bit compressive sensing, AR takes a different approach. It accounts for the lost amplitudes of the one-bit quantized measurements, and performs channel estimation and amplitude completion jointly. This way, the direction information of the propagation paths can be estimated via accurate direction finding algorithms in array processing, e.g., maximum likelihood. The upsot is that AR is able to handle off-grid angles and provide more accurate channel estimates. Simulation results are included to showcase the advantages of AR.

==> ar_spl copy/def.tex <==


\def\Re{\text{Re}}
\def\Im{\text{Im}}
\def\for{\text{for}}
\def\bbe{\boldsymbol{\beta}}
\def\bal{\boldsymbol{\alpha}}
\def\bga{\boldsymbol{\gamma}}
\def\bde{\boldsymbol{\delta}}
\def\bep{\boldsymbol{\epsilon}}
\def\bvep{\boldsymbol{\varepsilon}}
\def\bze{\boldsymbol{\zeta}}
\def\bet{\boldsymbol{\eta}}
\def\bth{\boldsymbol{\theta}}
\def\bvth{\boldsymbol{\vartheta}}
\def\bio{\boldsymbol{\iota}}
\def\bka{\boldsymbol{\kappa}}
\def\bla{\boldsymbol{\lambda}}
\def\bmu{\boldsymbol{\mu}}
\def\bnu{\boldsymbol{\nu}}
\def\bxi{\boldsymbol{\xi}}
\def\bo{\boldsymbol{o}}
\def\bpi{\boldsymbol{\pi}}
\def\bPi{\boldsymbol{\Pi}}
\def\bvpi{\boldsymbol{\varpi}}
\def\brh{\boldsymbol{\rho}}
\def\bvrh{\boldsymbol{\varrho}}
\def\bsi{\boldsymbol{\sigma}}
\def\bvsi{\boldsymbol{\varsigma}}
\def\bta{\boldsymbol{\tau}}
\def\bup{\boldsymbol{\upsilon}}
\def\bph{\boldsymbol{\phi}}
\def\bvph{\boldsymbol{\varphi}}
\def\bch{\boldsymbol{\chi}}
\def\bps{\boldsymbol{\psi}}
\def\bom{\boldsymbol{\omega}}
\def\bGa{\mathbf{\Gamma}}
\def\bDe{\mathbf{\Delta}}
\def\bTh{\mathbf{\Theta}}
\def\bLa{\mathbf{\Lambda}}
\def\bXi{\mathbf{\Xi}}
\def\bPh{\mathbf{\Phi}}
\def\bSi{\mathbf{\Sigma}}
\def\bUp{\mathbf{\Upsilon}}
\def\bPh{\mathbf{\Phi}}
\def\bPs{\mathbf{\Psi}}
\def\bOm{\mathbf{\Omega}}
\def\tr{\text{trace}}
\def\({\left(}
\def\){\right)}
\def\[{\left[\,}
\def\]{\,\right]}
\def\Nn{\nonumber}
\def\0{\boldsymbol{0}}
\def\1{\boldsymbol{1}}
\def\a{\mathbf{a}}
\def\A{\mathbf{A}}
\def\bA{\mathbb{A}}
\def\b{\mathbf{b}}
\def\B{\mathbf{B}}
\def\bB{\mathbb{B}}
\def\c{\mathbf{c}}
\def\C{\mathbf{C}}
\def\bC{\mathbb{C}}
\def\d{\mathbf{d}}
\def\D{\mathbf{D}}
\def\bD{\mathbb{D}}
\def\e{\mathbf{e}}
\def\E{\mathbf{E}}
\def\bE{\mathbb{E}}
\def\f{\mathbf{f}}
\def\F{\mathbf{F}}
\def\bF{\mathbb{F}}
\def\g{\mathbf{g}}
\def\G{\mathbf{G}}
\def\h{\mathbf{h}}
\def\H{\mathbf{H}}
\def\bfi{\pmb{i}}
\def\I{\mathbf{I}}
\def\j{\mathbf{j}}
\def\J{\mathbf{J}}
\def\k{\mathbf{k}}
\def\K{\mathbf{K}}
\def\l{\mathbf{l}}
\def\L{\mathbf{L}}
\def\m{\mathbf{m}}
\def\M{\mathbf{M}}
\def\n{\mathbf{n}}
\def\N{\mathbf{N}}
%\def\o{\mathbf{o}}
%\def\O{\mathbf{O}}
\def\p{\mathbf{p}}
\def\P{\mathbf{P}}
\def\q{\mathbf{q}}
\def\Q{\mathbf{Q}}
\def\r{\mathbf{r}}
\def\R{\mathbf{R}}
\def\bR{\mathbb{R}}
\def\s{\mathbf{s}}
\def\S{\mathbf{S}}
\def\t{\mathbf{t}}
\def\T{\mathbf{T}}
\def\cT{\mathcal{T}}
\def\u{\mathbf{u}}
\def\U{\mathbf{U}}
\def\bU{\mathbb{U}}
\def\v{\mathbf{v}}
\def\V{\mathbf{V}}
\def\w{\mathbf{w}}
\def\W{\mathbf{W}}
\def\x{\mathbf{x}}
\def\X{\mathbf{X}}
\def\y{\mathbf{y}}
\def\Y{\mathbf{Y}}
\def\z{\mathbf{z}}
\def\Z{\mathbf{Z}}
\def\De{\mathbf \Delta}
\def\Ze{\mathbf \Zeta}
\def\vec{{\mathrm{vec}}}
\def\mod{{\rm mod}}
\def\dUs{\bDe\U_s}
\def\Us{\U_s}
\def\Vs{\V_s}
\def\dVs{\bDe\V_s}
\def\Ls{\bLa_s}
\def\dLs{\Delta\bLa_s}
\def\Un{\U_n}
\def\Vn{\V_n}
\def\ha{\hat{\a}}
\def\hb{\hat{\b}}
\def\hR{\hat{\R}}
\def\hU{\hat{\U}}
\def\toep{{\mathrm{Toeplitz}}}
\def\snr{\text{SNR}}
\def\diag{\mathrm{diag}}
\def\sign{\mathrm{sign}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}


\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
